Enhancing Virtual Assistant Intelligence: Precise Area Targeting for Instance-level User Intents beyond Metadata

Virtual assistants have been widely used by mobile phone users in recent years. Although their capabilities of processing user intents have been developed rapidly, virtual assistants in most platforms are only capable of handling pre-defined high-level tasks supported by extra manual efforts of developers. However, instance-level user intents containing more detailed objectives with complex practical situations, are yet rarely studied so far. In this paper, we explore virtual assistants capable of processing instance-level user intents based on pixels of application screens, without the requirements of extra extensions on the application side. We propose a novel cross-modal deep learning pipeline, which understands the input vocal or textual instance-level user intents, predicts the targeting operational area, and detects the absolute button area on screens without any metadata of applications. We conducted a user study with 10 participants to collect a testing dataset with instance-level user intents. The testing dataset is then utilized to evaluate the performance of our model, which demonstrates that our model is promising with the achievement of 64.43% accuracy on our testing dataset.

==> 1-intro.tex <==
Have you ever complained about the virtual assistant on your smart devices? Since the first virtual assistant for smartphones, Siri, was installed on iPhone 4S in 2011 \cite{wikipedia_2022}, the last decade has witnessed the great convenience that virtual assistants brought to users' daily life. With their assistance, a vocal command of a user can replace a sequence of actions on screens to achieve a certain intent, e.g., `set an alarm at 6 AM', `check the weather today', `call Tom' etc. However, the provided services of virtual assistants are mainly based on built-in apps, covering a quite limited number of functionalities. Although platform-specific mechanisms such as Siri Shortcuts~\cite{apple_support_2020} and Android App Actions~\cite{android_developers} enable end-users to customize commands of virtual assistants for leveraging the exposed functionalities of installed apps, the exposed functionalities are heavily relying on the extra development efforts~\cite{uied}. If a user intent is out of its service scope, the virtual assistant will not fulfill the intent but show related websites or admit its incompetence instead. With the flourishing app market, it is crucial to narrow the huge gap between the rapidly growing user intents in various application scenarios and the limited functionalities supported by virtual assistants. 

User intent understanding and objective detection from user intents is another bottleneck that limits the ability of virtual assistants, which is the premise for providing target services for users. You may notice that assistants are not sufficiently capable of understanding and processing complicated user intents, e.g., instance-level user intents with details about scenarios. Actually, for human beings, there are tremendous ways to convey a purpose with diverse vocabularies, phrases, and grammatical structures, resulting in the set of possible user intents being intractable to be thoroughly pre-defined. To empower the virtual assistant to interact generally with installed apps, it thus is crucial to enable the assistant to handle user intents by finding the precise targeting operational area on screens of installed apps. 

Many existing works focused on augmenting the ability of virtual assistants ~\cite{r_10, r_24, r_28, r_46, r_49, r_58}.
An intuitive idea is to authorize the assistant with access to visit the metadata of installed apps. However, it still requires extra efforts from developers to make metadata readable for virtual assistants with developer overhead. Besides, the skill sets of assistants are still limited with the developer-declared built-in intents. The access to metadata may also cause privacy and security issues when the confidential information of users is exposed. Beyond the extra developing efforts, supervised learning based voice-to-action mapping is conducted in many existing works. However, the performance of machine learning based models requires a huge amount of intent-button labeled pairs, and the model may suffer from data noise caused during the labor-intensive data collection and labeling. Moreover, the capability of supervised learning models is trickily limited by the functionalities covered by the training dataset, while the whole model requires to be retrained for adding extra functionalities. 

To address these aforementioned problems, a capable model is required for thoroughly and accurately understanding the semantics of natural language expressed user intents together with the semantics of UI widgets on screens, and bridging the gap across the text and image modality. In this paper, we propose a novel pipeline leveraging natural language processing techniques and computer vision techniques to precisely target the operational area for instance-level user intents beyond metadata. Benefiting from the unsupervised learning adopted of our model, no built-in user intents are fed into the model such that the capabilities of models are not limited by a pre-defined service scope; no intent-button label data are required for model training such that existing datasets with high quality for natural language processing tasks or graphic processing tasks can be utilized and no extra labor-intensive data collection and labeling are required; no access requirement for metadata such that it is non-intrusive for private data of users; it can be generally adopted for installed apps without extra efforts from developer or end-users.

During the offline steps of our model, we fine-tuned an advanced natural language processing model, Bert~\cite{devlin2018bert}, with textual user manuals for mobile apps, which is deployed for user intent understanding and user objective prediction. We also trained an icon classifier using a cleaned icon dataset captured from the Kaggle website~\cite{test.ai_2018} to standardize icon labels for cross-modality matching, which currently supports 80 icon classes, but can be extended with other mobile icon datasets. With the descriptive words and images data from nounproject, we utilized the icon classifier to print a label for each image and stored the descriptive word and label pairs in a generated local database. We also proposed 13 voting algorithms for merging the results to determine the most likely icon label to be searched in the following online steps. By online steps, given the natural language user intent, the BERT-based MLM model is adopted to predict descriptive words for the targeting operation area with corresponding probabilities. Specifically, for each input user intent for our model, we designed prompt templates by adding a sub-sentence to the original user intent. For example, for the user intent, `I want to add this phone to my favourites', the input for the Bert MLM model after processing would be `I want to add this phone to my favourites, so the [MASK] icon should be clicked.`. The Bert model then predicts relative words that are most possible to replace the location of `[MASK]', which can be regarded as descriptive words for the targeting area. The generated descriptive words are then processed by a Descriptive-Words Classifier, producing several local labels for the list of descriptive words, where the Descriptive-Words Classifier is composed of a local database and a group of voting agents as referred to in the offline steps. Next, we leveraged GUI detection tool UIED~\cite{uied} for detecting graphic and textual elements on the user screen, where for each detected graphic element, we adopted the icon classifier to predict a local label. Finally, the precise targeting operational area is determined by matching the targeting labels predicted by the Descriptive-Words Classifier with predicted labels of detected graphic elements as well as the textual elements. A flowchart of our model is illustrated in Fig.~\ref{fig_flow_chart}.

For the evaluation of our model, we conducted a user study for collecting testing datasets with the various user intents and ground truth of the operational area. To ensure data diversity, representativeness, and completeness, the testing UIs are selected from ranked app categories of App Store on iPhone, iPad, and Mac. Overall, we downloaded 198 apps in total, among which 66 apps are on iPhone, 69 apps are on iPad and 63 apps are for Mac which are ranked in top 1, top 20 and a randomly selected rank. Within the downloaded, we selected UIs with different layouts, elementary component types, component numbers, color themes, etc. We
recruited 10 participants with gender diversity, from different countries, at different ages and different working positions. To test the capability of our model under the scenarios where the annotations about buttons are not available, we augmented the testing database with mosaic processing on the annotation of selected UIs. The accuracy of our model on the collected testing UIs is $64.43\%$ and the accuracy on the collected UIs with the positive Mosaic UIs is $58.56\%$.

The contributions of our work are listed as follows.
\begin{itemize}
    \item We proposed a novel problem to empower the virtual assistant to generally interact with installed apps, with the ability to precisely target operational areas for instance-level user intents without access to metadata.
    
    \item To the best of our knowledge, we are the first to adopt the Bert MLM model for thoroughly understanding user intents and accurately detecting user objectives, while precisely predicting descriptive words for targeting areas.
    
    \item We designed a novel pipeline through unsupervised learning combining natural language processing techniques and computer vision techniques, without built-in intents and intent-button training dataset required.
    
    \item We collected a dataset with diversity, representativeness, and completeness, containing instance-level user intents and precise targeting operational areas on iOS UIs for testing automation. 
    
\end{itemize}

==> 2-related_work.tex <==

\section{Related Work}
In this section, we will introduce virtual assistants, shortages of virtual assistants and design goals for our approach.

\subsection{Virtual Assistants}

Virtual assistants like Siri for iOS and Google Assistant for Android have been widely adopted in tremendous smart devices. They support users with hands-free and eyes-free interactions, automatically dealing with everyday tasks through simple voice commands from users~\cite{wulf2014hands, zhong2014justspeak, arsan2021app}. However, the provided services of virtual assistants are mainly based on built-in apps, covering a quite limited number of functionalities. The exposure of the capabilities of installed apps to virtual assistants requires extra manual efforts from developers. Even when developers pay a great number of efforts to enable installed apps to be leveraged by virtual assistants, there are still many limitations for both Android and iOS platforms~\cite{uist}. 

\subsection{Shortages of Virtual Assistants}

Only a limited number of built-in intents are supported by Google Assistant~\cite{uist}. To enable an installed app to interact with the Google Assistant, developers of the installed app can use App Actions~\cite{android_developers} to add extra file (actions.xml) to declare the exact built-in intents that can be leveraged. These built-in intents are pre-defined in Android system, and cannot be expanded by developers of installed apps. The Google Assistant thus cannot automatically help for processing custom tasks which are out of the scope of built-in intents. For example, `find videos posted nearby' for social media apps like TikTok, `check booking history' for reservation apps like Booking.com and `update Covid-19 vaccine record' for health apps are not able to be processed by Google Assistant. Although the built-in intents list can be expanded by developers of Android system, it will require a huge amount of manual efforts for investigating the custom capability of apps in the rapidly growing app market, and updating related system documents. 

Siri on iOS can also interact with installed apps in a similar way to Google Assistant, where an Intent Definition File which declares the capabilities of an app is required (i.e., iOS intents)~\cite{uist}. Moreover, Siri also enables developers to encode custom intents, where developers need to define a mechanism that donates the shortcut to Siri every time the user intent is supported ~\cite{apple_developer_documentation, uist}. Developers can also link app functionality to Siri via suggested Shortcuts~\cite{apple_support_2020}, which requires manual configuration from end-users.

Even when great manual efforts from developers and even end-users are made, the added intent file or edited shortcut is app-specific, which serves a certain app and cannot be automatically adopted to other apps with similar functionalities. For example, almost all weather apps have the functionality of `check weather'. Instead of effectively reusing a completed intent file of other apps, developers of all weather apps need to add intent files for their own app in order to expose the functionality to the virtual assistant, although intent files of different weather apps could be quite similar. Moreover, the capabilities exposure of installed apps is also platform-specific. For the same app that serves on different platforms like iOS and Android, developers of the app should make efforts on interacting with different virtual assistants respectively. For example, to enable the intent `open dialogue using Whatsapp' to be interfaced by both Siri and Google Assistant, developers of Whatsapp should edit intent-related files on both iOS and Android. 

Moreover, to the best of our knowledge, virtual assistants only have app-level access to installed apps, which treats a certain app as a tool to complete a specific task for end-users, for example, sending money, setting an alarm, playing music, etc. In contrast, many everyday tasks are on UI-level, which heavily relies on certain UI contents. For example, `thumb up for this post' (on UIs displaying certain posts of social media apps), `Send video call' (on UIs displaying chatting dialogues of message apps), `Set this message into unread status' (on UIs displaying certain e-mails of mail apps). The UI-level user intents thus can not be processed by current virtual assistants.

\subsection{Design Goals of our Model}

By the observation of the limitations of current virtual assistants, we proposed multiple design goals for our virtual assistant in this paper: 1) zero-effort is required from both developers and end-users to expose app capabilities to the virtual assistant; 2) the virtual assistant is cross-app and cross-platform; 3) the virtual assistant is capable for custom tasks and UI-level tasks. Apart from tackling the aforementioned limitations, we also set extra design goals to further enhance the capabilities of virtual assistants: 4) thoroughly and accurately understand instance-level user intents; 5) precisely find the targeting operation area of user intent; 6) based on UIs only without any metadata of apps to protect privacy and security of end-users.





==> 4-model.tex <==
\section{Approach}
\label{sec_approach}
In this section, we will introduce our model architecture in details.

\subsection{Model Architecture}

The input of our model is a screenshot together with an instance-level vocal or textual user intent, where details of the user objective are clarified. We designed a novel deep-leaning pipeline model to solve the problem. 

Our model firstly understands and detects the intent from the natural language, and predicts the most possible words of the target button names in general language together with the corresponding possibilities, utilizing the Masked Language Model of Bert~\cite{devlin2018bert}. The predicted words by Bert are then transmitted to local labels owning to a local 80-class label list via a word-to-label translation agent. The agent also calculates the searching priorities for the recommended local labels through multiple voting algorithms. The output by the word-to-label translation agent is the target labels to be searched over the screen.

On the other hand, all icons and texts on the input screens are detected and captured via a GUI elements detection toolkit UIED~\cite{xie2020uied}. The captured icons then go through an icon classifier to be identified as a set of local labels owing to the aforementioned local 80-class label list. The target labels recommended by the word-to-label translation agent are then searched among the set of labels predicted by the icon classifier one by one according to their priorities in descending order. 

If all target labels are not found among the predicted labels from icons, the text contents on the input screen detected by UIED are considered. Each distinct word in the textual user intent is recognized as a token for text searching. The words predicted by Berts as well as the target local labels recommended by the word-to-label translation agent are also regarded as tokens. The identified tokens are then searched over the text contents detected on the screen, where the number of tokens contained in each text area is counted and the text area with the largest number of tokens is identified as the target operating area for the user intent.


\subsection{User Intent Detection and Prediction}


Our task is to detect the target operational button on an input screen for the user intent. Different from the object detection tasks of computer visual field, where the input user intent is a determined `label', the task studied in this paper requires our model to leverage the natural language description of user intent to find the goal of the user intent, i.e., what does the user want to do. It should also provide hints for the target area, i.e., where to click to achieve the goal of the user. 
Different from the high-level user intents, e.g., `send money', `set an alarm', `listen to music' \cite{arsan2021app}, the instance-level user intent contains more details of the practical scenarios, e.g., `I wish to check what I have added into the trolley', `I am interested in fashion and would like to dive deep into that category', and `I am trying to find what translation records I have saved for future use'. There are various ways to state a user intent. For example, with the aim of speaking during an online meeting, people may say `I want to speak', `I wish to unmute myself', 'I would like to use my microphone' etc. The flexibility of the natural language expressions with various statements, sentence structure, grammatical modifiers, and other components thus makes the set of user intents an infinite one, which cannot be processed directly as a classification problem like most high-level intent tasks do. Instead, our model should be able to detect the intent from the instance-level description, and produce some hints or predictions for the target operational area. For example, for the aim of speaking over the online meeting, the target operational area is related to `voice' according to our experience of mobile application usage. And the hints of the target operational area thus help to focus on related icons among various components over the screen. 
 
A capable natural language processor which has rich experience in mobile applications is preferred. However, there is no existing model with the ability to predict an operational target area for user intent. Our inspiration is from the training process of Bert (Bidirectional Encoder Representations from Transformers) \cite{devlin2018bert}, which applied Masked Language Model (MLM) by randomly masking 15\% of all WordPiece tokens in each sequence of the input sentence and predicting the masked vocabulary id relying only on the context. It indicates that Bert is advanced in predicting a masked word in a sentence. For example, for a given sentence with a special mark `[MASK]' inside, the MLM of a pre-trained Bert regards the `[MASK]' as a missing vocabulary, and is able to predict a list of words with corresponding possibilities. Besides, since Bert is trained on a huge amount of textual materials, it is `knowledgeable' enough to provide suggestions for many queries it has `learned' before. For example, for the sentence `The capital of the UK is [MASK].', the most possible  5 vocabularies predicted by Bert (`bert-base-uncased' version) are `london' with probability 0.265, `manchester' with probability 0.094, `edinburgh' with probability 0.070, `birmingham' with probability 0.060 and `bristol'with probability 0.034 \cite{DBLP:journals/corr/abs-1810-04805}.

The Bert model we deployed in our model is  'bert-base-uncased', which is pre-trained on a dataset called BookCorpus, with 11,038 unpublished books and English Wikipedia (excluding lists, tables, and headers)\cite{DBLP:journals/corr/abs-1810-04805}. It is case-insensitive, e.g., it does not make a difference between `english' and `English'. We choose it since its training dataset is capable enough to learn an inner representation of the English language\cite{DBLP:journals/corr/abs-1810-04805}. To let the Bert model gain expertise on mobile application guidelines, we fine-tuned the Bert model with 50 mobile application handbooks downloaded from official websites of mobile applications. Taking advantage of the prediction ability of Bert, we applied Bert in a novel way to provide hints for the target operational button, by joining the original user intent with the text --- \textit{', so the [MASK] icon should be clicked.'} For example, if the original user input is `I wish to check what I have added into the trolley', the input for the Bert model would be `I wish to check what I have added into the trolley\textit{, so the [MASK] icon should be clicked.}'. As a result, Bert would output a list of candidates for the `[MASK]' unit with corresponding possibilities in descending order. We take the top 5 vocabularies predicted by Bert as the input for the next step. Note that, our model can process English user intent only. All vocal user intents will be first transformed to text by `speech-to-text' technology.

\subsection{Element Detection and Classification on Screen}

With the vocabulary predicted by Bert, it is intuitive to find the components on the screen which are related to the provided descriptive words. However, unlike human beings who are enabled by instincts to distinguish different items in an image, on the perspective of computers, images are just combinations of massive pixel values, without any sense of displayed objects. To find the targeting button, our model thus should have the ability to identify various components on a screen. 

We applied User Interface Element Detection (UIED)~\cite{uied} to detect elements on the input screen. UIED is a toolkit designed for GUI element detection. By utilizing UIED, the locations of both the graphic content and the textual content on a screen are detected.

For the detected graphic elements, we trained a CNN icon classifier to generate a label for each icon based on its pattern. The training dataset is derived from icon images on the `Common Mobile/Web App Icons' from the Kaggle website \cite{test.ai_2018}, which contains 106 classes, with 153380 images. The Kaggle dataset also contains a 'negative' class with 10564 images which do not belong to any other 105 classes. Since the Kaggle dataset is designed for both web and mobile Apps, there are some unsuitable categories for our tasks. For example, icons in the `cursor' category rarely appear on mobile screens, we thus remove these categories from the training dataset. Besides, the biggest problem with utilizing the dataset is that, as claimed in the description on the official website of the `Common Mobile/Web App Icons' dataset, there are many icons in the wrong categories. For example, there are a large number of images of `arrow right', `arrow up', and `arrow down' contained in the category of `arrow left', which significantly limits the capability and performance of the classifier, we thus manually cleaned the images in each category and moved the images with incorrect labels into the correct category. Considering the detected graphic elements are likely to contain images that are not for clicking purposes, e.g., background images, profile pictures, images inserted into textual content, or illustrative diagrams, we kept the category `negative' to distinguish these image contents from normal icons. After the manual data cleaning, the number of images used for the classifier is 26970 in 80 categories, with 79 icon classes and 1 `negative' class.

We trained an 8-layer CNN model with 1000 hidden neurons as the icon classifier, with a momentum of 0.5 and kernel size of 5, with a batch size of 64 for 30 epochs, which achieved the best performance compared with models with other experimental settings under the constraint of our hardware device (i9-10900k CPU and GeForce RTX 3090 GPU with 24G memory). It reached 95.57\% accuracy on the testing dataset. With the icon classifier, the graphic elements detected by UIED are classified into one of 80 categories. As a result, each graphic element that resembles a mobile icon is predicted with one of the labels from the 79 icon classes based on its pattern, while the ones similar to images in the content are labeled as `negative'.   

For the textual elements on the screen, both their locations and textual contents are captured by UIED, which are also utilized for identifying the target operational icon in the following steps.

\subsection{Cross-Modality Bridging}
On the one hand, the natural words predicted by Bert provide hints of the target operational button. On the other hand, the elements on the screen detected by UIED present a list of candidates for the target operational button, which includes both graphic elements and textual elements. In the following, we will show a novel cross-modality bridge to find the element that best aligned with the descriptive words delivered by Bert, where the graphic elements and textual elements detected by UIED are searched respectively. 

\subsubsection{Search in Visual Elements}
We want to find the visual elements which align best with hints from Bert. Note that, the descriptive words provided by Bert are all about the functions of the desired buttons, instead of their patterns. 

With the aforementioned icon classifier, each graphic element detected by UIED is predicted with one label among the 80 local classes. We ignored the elements with the `negative' label, since they are not regarded as normal buttons by the icon classifier. To find the target button, it is intuitive to measure the similarity between the label of each detected graphic element and the descriptive words produced by Bert. However, this intuitive approach highly depends on the linguistic contents of labels, which may result in significant bias. To be specific, predicted labels of graphic elements come from the names of categories of the training dataset, which are used as symbols to distinguish images of one class from images in other classes. The names of categories are not compulsorily related to the content of images inside each category, e.g., numerals are commonly used as labels for many classification tasks. Even though labels can be manually replaced by words related to the content of images in each category, it is unlikely to find a word to absolutely and precisely describe the functions of images in each category. For example, the natural words 'cart', 'shop', 'buy' and 'purchase' can all represent the category of icons related to shopping. For the user intent `I wish to purchase a new umbrella', one descriptive word predicted by Bert is `Store'. There is an icon with the `shopping cart' pattern on the screen to present the purchasing function and an icon with a `house' pattern to represent the home page. If we choose `cart' as the label of the category corresponding with shopping, and choose `house' as the label of the category corresponding with images containing house patterns, the `house' icon is likely to be selected as the target button rather than the desired button with the shopping cart pattern, due to the higher similarity of the word `house' than the word `cart' by some similarity measurement models. 

To solve the problem, we designed a Descriptive-Words Classifier to classify the predictive words predicted by Bert with one or multiple labels from the local 80 labels, totally beyond the linguistics of labels. The local 80 labels are exactly the same as the labels produced by the icon classifier.

Our initial approach of the Descriptive-Words Classifier is that, given a natural descriptive word of a category of icons, e.g. `alarm', we first let the classifier know the appearance of these kinds of icons by automatically downloading a certain amount of images with the keyword `alarm icon' through online searching engines. We then unitize the aforementioned icon classifier to predict a label for each downloaded image. In this way, the model downloaded images for each word predicted by Bert, with a list of labels predicted by the classifier. All the predicted labels by the icon classifier are ordered descendingly based on their frequencies, which are the output of the Descriptive-Words Classifier as the labels for the descriptive words of Bert. This approach works well for many user intents. However, the biggest problem of this approach is that the running time of each user intent is more than 20 seconds due to the downloading speed limited by online search engines, which are inefficient to be adopted for real applications. To improve the running speed and accuracy, we upgrade the approach by replacing the online search engine with a local dataset with multiple voting agents for selecting the output labels.

The upgraded Descriptive-Words Classifier combined a local dataset with 13 voting agents, where each voting agent votes for one or multiple labels based on its own voting algorithm. The labels ordered descendingly based on their votes are as the output. The detailed structure of the Descriptive-Words Classifier is as follows. 

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{Figs/noun_project.jpg}
    \caption{An illustrative example of the source of data in the generated local database.}
    \label{fig_noun_project}
\end{figure*}

The local dataset is generated from the data of nounproject, which contains information on icons including names, designers, searching words for related icons and etc, where searching words are keywords to find the corresponding icon~\cite{noun_project}. As shown in the left table in Fig.~\ref{fig_noun_project}, where each image is with multiple natural words as the searching words. For example, the icon in the first row has four keywords: `Arrow', `Play', `Movie' and `Next'. Note that, there are various icon images with quite similar patterns but with different keywords, e.g., the icons in the third and the fourth rows. 

To generate the local database, we utilized the aforementioned icon classifier to predict a label for each icon image. As a result, each icon image of the noun project database is predicted with a local label among the 80 classes. For example, the icon listed in the first row of the table is predicted with the local label, `arrow\_right'. Regarding the image of the icon as an intermedium, we thus got four word-label pairs, i.e., (`Arrow',`arrow\_right'), (`Play', `arrow\_right'), (`Movie',`arrow\_right') and (`Next', `arrow\_right') respectively. These produced word-label pairs are inserted into the local database for statistical purposes. $1,547,847$ images from the noun projects are utilized and there are $6,348,857$ descriptive words in total, among which the number of distinct words is $214,377$. Consequently, there are $6,348,857$ word-label pairs stored in the local dataset. Fig.~\ref{fig_cloud_word} shows a word cloud containing the top 100 descriptive words with the highest frequency of the database, where the larger the fonts of words are, the higher frequencies they are with. Fig.~\ref{fig_bar_label} presents the top 20 labels with the most descriptive words stored in the database.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figs/fig_Cloud_Word_top100.png}
    \caption{The Word Cloud presenting the top 100 descriptive words with the highest frequencies in the local database.}
    \label{fig_cloud_word}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figs/fig_bar_label_count.png}
    \caption{The top 20 labels with the most descriptive words in the local dataset. }
    \label{fig_bar_label}
\end{figure*}
With the predictive words predicted by Bert together with the possibility of each word, we wish to utilize the local database to find a local label that is the closest to the provided predictive words. There are various strategies to match the local labels, where strategies focusing on different features may prefer different local labels. For example, the 5 words predicted by Bert are 'call', 'phone', 'user', 'contact', and 'talk', with probabilities for each word. One strategy is that, find all word-label pairs inside the database where the descriptive word is among these given 5 words, and find the local label with the highest frequency as the final selected local label. One of another strategy is that, for each of the 5 words, select the local label with the highest frequency pairing with this descriptive word in the database, e.g., the local labels selected for `mobile', `phone', `user', `contact' and `talk' are `call', `call', `user', `file' and `volume' respectively, where the number of the appearance of the local label `call' is 2, which is the largest among the appearance numbers of the other 3 labels, the local label `call' thus is selected as the final local label. Both of the mentioned 2 strategies are feasible, but may produce different outputs as the final selected local label. Furthermore, both strategies highly depend on the composition of the data source of the local database, e.g., changing data sources with more pairs of certain descriptive words or local labels will affect the decision-making of different strategies to different degrees. To improve the generalization ability by selecting the local label beyond the composition of the data source, we thus designed a group of voting agents focusing on different features (including 8 deterministic algorithms and 5 non-deterministic algorithms) to improve the fairness and mitigate the biases caused by the data source. The details of each voting algorithm are as follows.

For Approaches 1.1, 1.2 and 1.3, for each word predicted by Bert, we first find a local label candidate for each of the words, which is the one with the highest frequencies paired with the word in the database. For example, for the input of the Bert, `If click the [MASK] icon, it adds the item to the shopping trolley.'  We can get these descriptive words predicted by Bert: $w_1 = 'item'$ with probability $p_1 = 0.217$, and $w_2 = 'store'$ with $p_2 = 0.0759$, $w_3 = 'shopping'$ with $p_3 = 0.0497$, $w_4 = 'product'$ with $p_4 = 0.0415$, $w_5 = 'purchase'$ with $p_5 = 0.0374$. When we input $w_1 = 'item'$ as a descriptive word into the database, we can find $3,058$ word-label pairs with 'items', among which the word-label pair with the highest frequencies are ('item', 'airplane'), with $128$ appearances among the $3,058$ pairs, we thus get the percentage $q_1$ of $'(w_1, l_1)'$ pair among all $w_1$ related pairs as $q_1 = \frac{128}{3058} = 4.186\%$. In the same way, we can get the related labels and percentages for $w_2, w_3, w_4$ and $w_5$ respectively, which are $l_2 = 'cart'$ with $q_2 = 16.882\%$, $l_3 = 'cart'$ with $q_3 = 26.298\%$, $l4 = 'barcode'$ with $q_4 = 7.617\%$ and $l5 = 'cart'$ with $q_5 = 22.665\%$. So far, we have got $5$ local label candidates together with their percentages. 
\begin{itemize}
\item {Approach 1.1: Only focus on the 5 label candidates from $l_1$ to $l_5$, vote for the one with the maximum appearances among the $5$ labels. 

\textit{In this case, there are 3 distinct labels, `airplane’, `cart’ and `barcode’, with the number of appearances $1$, $3$ and $1$ respectively. So the label with the maximum appearance is ‘cart’, which gets one vote from Approach 1.1.}}

\item Approach 1.2: For each distinct label $l'$ from $l_1$ to $l_5$, find its accumulated percentage $f(l') = \sum_{ l_k = l'}q_k$ and vote for the one with the maximum $f(l')$ value.

\textit{In this case, there are 3 unique labels, `airplane’, `cart’ and `barcode’, with
$f('airplane') = q_1 =4.186\% $; $f('cart') = q_2 + q_3+ q_5 =16.882\% + 26.298\% +22.665\% =65.845\%$; $f('barcode') = q_4 =7.617\%$. So the label with the maximum  $f(l')$ value is $‘cart’$, which gains one vote from Approach 1.2.}

\item Approach 1.3: For each distinct label $l'$ from $l_1$ to $l_5$, find the accumulated value of its probability multiplies its percentage $g(l') = \sum_{l_k = l'}p_k\times q_k$, where probability is provided by Bert. Vote for the candidate label with the maximum $g(l')$ value.

\textit{In this case, $g('airplane') = p_1q_1 = 0.908\%$; $g('cart') = p_2q_2 +p_3q_3+ p_5q_5 =3.436\% $; $g('barcode') = p_4q_4 =0.316\%$. So the label with the maximum $g(l')$ value is ‘cart’, which gains one vote from Approach 1.3.}
\end{itemize}
For the following approaches, a local label candidate corresponding with each word predicted by Bert is no longer required.
\begin{itemize}

\item Approach 1.4: For each word $w_k$, find all labels $l_k^m$ paired with $w_k$, together with the count $c_k^m$ of the label $l_k^m$ stored in the data set. Select the label $l'$ with the maximum count $c'$.

\textit{In this case, the $5$ words are `item’, `store’, `shopping’, `product’ and `purchase’. Among word-label pairs containing any one of these $5$ words, the frequencies of local labels in non-increasing order are: $3,911$ for `cart', $2,117$ for `bag', $932$ for `dollar' ... , where `cart', `bag' and `dollar' are local labels. The label ‘cart’ with the maximum number $3,911$ of images thus gains one vote from Approach 1.4.}


\item Approach 1.5: For each word $w_k$ provided by Bert, find all labels $l_k^m$ paired with $w_k$, together with the percentage $q_k^m$ that label $l_k^m$ stored in the dataset. The label $l'$ with the maximum percentage $q'$ gains one vote from Approach 1.5.

\textit{In this case, the label ‘cart’ with the maximum sum of percentage $0.7334$ is selected. }

%mean value

\item Approach 1.6:  For each distinct label $l'$ from $l_1$ to $l_5$, find its averaged accumulated percentage $f(l') = avg(\sum_{l_k = l'}  q_k)$. Vote for the one with the maximum $f(l')$ value.

\textit{In this case, there are $3$ distinct labels, `airplane’, `cart’ and `barcode’, with
$f('airplane') = q_1 =4.186\%$; $f('cart') = \frac{q_2 + q_3+ q_5 }{3} =\frac{16.882\% + 26.298\% +22.665\% }{3} =21.948\%$; $f('barcode') = q_4 =7.617\%$. So the label with the maximum  $f(l')$ value is ‘cart’, which gains one vote from Approach 1.6.}

\item Approach 1.7: For each unique label $l'$ from $l_1$ to $l_5$, find the averaged accumulated value of its probability multiplies its percentage $g(l') = avg(\sum(l_k = l')  p_k\times q_k)$. Vote for the one with the maximum $g(l')$ value.

\textit{In this case, $g('airplane') = p_1q_1 = 0.2174.186\% = 0.908\%$; $g('cart') = \frac{p_2q_2 +p_3q_3+ p_5q_5}{3}=1.145\%; \ \ \ \ \ \ \ \ \ \ $ 
   $g('barcode')=p_4q_4 =0.04157.617\% =0.316\%$. So the label with the maximum $g(l')$ value is ‘cart’, which gains one vote from Approach 1.7.}

\item Approach 1.8: For each word wk, find all labels $l_k^m$ together with the percentage $q_k^m$ label $l_k^m$ stored in the dataset. Select the label $l'$ with the maximum averaged accumulated percentage $q'$. 
\end{itemize}

The non-deterministic approaches are that: for each word $w$ from $w_1$, $w_2$, $w_3$, $w_4$ and $w_5$ predicted by Bert, Approach 2.1 randomly select $10$ word-label pairs containing $w$. Vote for the label with the highest frequency among the $10$ selected pairs. Approach 2.2, 2.3, 2.4 and 2.5 act similarly to Approach 2.1, where the only difference is that the number of pairs randomly selected for Approach 2.2, 2.3, 2.4 and 2.5 are $20$, $50$, $100$, and $200$ respectively.

Each voting approach votes for one local label (vote for multiple labels only when the voted multiple labels equally meet the requirement of an approach). As a result, the local labels with at least one vote are ranked based on the number of their received votes non-increasingly. The voted local labels in descending order are presented as the output of the Descriptive-Word Classifier, for the descriptive words provided by Bert. For example, the local label voted by approaches from 1.1 to 1.8 and approaches from 2.1 to 2.5 is `cart'(voted by Approach 1.1), `cart'(voted by Approach 1.1), `cart'(voted by Approach 1.1), `cart'(voted by Approach 1.2), `cart'(voted by Approach 1.3), `cart'(voted by Approach 1.4), `cart'(voted by Approach 1.5), `cart'(voted by Approach 1.6), `cart'(voted by Approach 1.7), `cart'(voted by Approach 1.8), `bag'(voted by Approach 2.1), `dollar'(voted by Approach 2.2), `barcode'(voted by Approach 2.3), `bag'(voted by Approach 2.4) and `cart'(voted by Approach 2.5). So for the input, descriptive words predicted by Bert: $w_1 = 'item'$ with probability $p_1 = 0.217$, and $w_2 = 'store'$ with $p_2 = 0.0759$, $w_3 = 'shopping'$ with $p_3 = 0.0497$, $w_4 = 'product'$ with $p_4 = 0.0415$, $w_5 = 'purchase'$ with $p_5 = 0.0374$, the output of the local label are (`cart', `bag', `dollar', `barcode'). 
Recall that, for each graphic element detected by UIED on the screen, it is predicted with one of the local labels by the Icon Classifier. To find the target graphic element, we first search elements to find the one or multiple with the predicted label with the highest priority, which is `cart' in the mentioned case. If the label with the highest priority cannot be found among the detected graphic elements, the label with the secondly highest priority is then searched, and so on, until a graphic element with the desired label is found, which is regarded as the target operational button. If none elements detected are with any label in the output of the Descriptive-Word Classifier, the textual elements detected by UIED are utilized.     

\subsubsection{Search in Textual Elements}

By previous steps, for each user intent, textual hints about the target area include 3 parts: 1) the original user intent (a textual sentence transformed from user voices); 2) descriptive words predicted by Bert, and 3) the labels predicted by the aforementioned Descriptive-Word Classifier. Each distinct word in the 3 kinds of hints is regarded as a token. For example, the user intent is `I plan to add the item to the shopping'; input the user intent to Bert, the descriptive words predicted by Bert are `item', `store', `shopping', `product' and `purchase'; input the words predicted by Bert to the Descriptive-Word Classifier, the labels predicted by the classifier are `cart', `bag', `dollar', `barcode'. The distinct words of these 3 groups of tokens are: `I', `plan', `to', `add', `the', `item', `shopping', `item', `store', `product', `purchase', `cart', `bag', `dollar', `barcode'. Then remove non-meaningful tokens e.g., `to' and `the', since they may appear multiple times in content on the screen, which may result in unsuitable results predicted by our model. The remaining words are searching tokens to find in each text piece detected on the screen. Count the number of tokens covered in each textual element. Then the textual elements containing more tokens are with higher priority to be highlighted on the screen. 

==> 5-user_study.tex <==
\section{User Studies}
There is no existing dataset on the public with instance-level user intents that could be utilized for testing our model. To evaluate the performance of our model, we thus conduct a user study to collect testing data from volunteers, who have experience using smartphones for more than 5 years. To access the capabilities of handling the user intents in practical scenarios, we simulate the user interactions in real-world circumstances with screenshots collected from free apps of each ranked category on the App Store (Australia) with a certain regulation. Users in different groups may have different understandings of icons displayed on screens, and they may also have different expressions on their intents, we thus investigated users including both males and females, who are distributed in 5 different age groups, living in 5 different countries, speaking 5 different languages in total, with 6 different positions. During user studies, volunteers are required to observe testing screens and propose user intents based on their own understanding of semantics of icons displayed on screens. Users also rated the alignment between their expectations of selected icon patterns and the text content of those icons. The user intents provided by users are collected and annotated as a testing dataset to automatically evaluate the performance of our model. 

\subsection{Diversity of Participants}
The main purpose of the user study is to collect testing data from users to evaluate the performance of our model in practical applications. The user intents provided by each user are not only relied on their understanding of icon semantics, but also on their own styles of expressing their intents via natural languages.

For the part of semantic understanding, due to the fact that there is no standard textbook teaching people which icons should match which functionalities, people acquire senses of icon understandings mainly from their own experience during app explorations. It thus implies that when users with diverse app experiences look at the same icon patterns, they may have distinct ideas. The living country is a crucial factor that has an impact on the user's comprehension of icon semantics. For example, apps vary significantly among different regions of App Stores, including the functionalities and design styles of each app. Gender, age, and positions are also factors that have unneglectable effects on users' most frequently used apps. On the aspect of natural language styles of expressing user intents, except for the aforementioned factors, the effects of languages spoken by users can not be ignored either.

Considering the mentioned issues above, we invited 10 people who have been using smartphones for more than 5 years to participate voluntarily in our user studies. 
The 10 participants are currently living in 5 different countries, i.e., Australia, Canada, China, the United Kingdom, and the United States (listed in alphabetical order), with 2 females and 8 males. The distribution of user ages is shown in Fig.~\ref{fig_pie_user}, with a minimum age of 23 and the maximum age of 56. The positions of participants include students, algorithm scientists, research fellows, technical sales, and financial analysts. Users can speak 5 languages in total, i.e., English, Chinese, Japanese, Korean and Russian. Nevertheless, all users are fluent in using English.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figs/fig_user_pie_chart.png}
    \caption{Age distribution of user study participants.}
    \label{fig_pie_user}
\end{figure}



\begin{comment}
\begin{table}[ht]
    \caption{Distribution of Participants' Ages \jieshan{I think a pie chart is more appropriate. see https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9402139 Figure 3?}
    }
    \centering
    
\begin{tabular}{ |c|c|c| } 
 \hline
 Age Group& Number of People & Percentage \\ 
 \hline
 15-24 & 3 & 30\% \\ 
 \hline
 25-34 & 3 & 30\% \\ 
 \hline
  35-44 & 2 & 20\% \\ 
 \hline
  45-54 & 1 & 10\% \\ 
 \hline
  55+ & 1 & 10\% \\ 
 \hline
\end{tabular}
\label{table_age}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[ht]
    \caption{Contact Information of Participants \jieshan{No need to add this table. You can just elaborate some demographic background of the participates, such as ages, gender and experience of using Mobile apps}
    }
    \centering
\begin{tabular}{ |l|l| } 
 \hline
 Participant Name & Contact Info  \\ 
 \hline
  Artem A. Lensky & artem.lensky@anu.edu.au\\
 \hline
  Jiaxu Liu  & jiaxu.liu@ieee.org\\ 
 \hline
  Matthew Aitchison & matthew.aitchison@anu.edu.au\\
 \hline
 Mengyan Zhang & mengyan.zhang@anu.edu.au\\
 \hline
 Ruikai Cui & ruikai.cui@anu.edu.au\\ 
 \hline
 Xueyuan Bai & baixueyuan@hotmail.com\\
 \hline
  Xuezheng Bai & xzbai@yahoo.com\\
 \hline
 Yang Liu & yang.liu3@anu.edu.au\\ 
 \hline
 Yukang Liu & yukang\_liu@sfu.ca\\ 
 \hline
 Zhenyue Qin & zhenyue.qin@anu.edu.au\\ 
 \hline
\end{tabular}
\label{table_user_info}
\end{table}
\end{comment}

\subsection{App Screen Collection}

To evaluate the capability of our model for handling tasks in real virtual assistants scenarios, we explored free apps in each ranked category of Apple Store on iPhone, iPad and Mac respectively. Since our model can only recognize user intents in English, we thus select a region in App Store with English as the official language. Although our model is capable to process tasks based on icons on screens without utilizing the text contents, characters in other languages like Chinese or Korean are easily recognized as icon patterns, which reduces the performance of icon recognition. The advanced model that can handle other languages will be considered in our future study. Due to the limitations that many explored apps in App Store (US) require American telephone numbers for registration, we are unable to explore many downloaded apps. We thus choose our living country as the region for the App Store.

We explored all free ranked categories in App Stores on iPhone, iPad, and Mac. For the App Store on iPhone, there are 28 categories in total, among which `Apple Watch Apps', `AR Apps', `Developer Tools', `Graphics \& Design', and `News' these 5 categories don't have an official ranked list and the category `Safari Extension' is for web page function extensions, which is not suitable for our tasks. We thus explored the remaining 22 categories for screen collection. The `News' category is ranked on iPad App Store, we thus explored 23 categories for iPad. Different from iPhone and iPad, there are 21 categories in total on the Mac App Store, and all of these 21 categories have an official ranked list. Overall, we downloaded 198 apps in total, among which 66 apps are on iPhone, 69 apps are on iPad and 63 apps are for Mac.

For each of the aforementioned free and ranked categories, we downloaded and installed the top 1, the top 20, and a randomly selected app on the ranked list respectively. Apps on iPhone and iPad are downloaded on 28th Feb 2022, while apps on Mac are downloaded on 11th March 2022. Note that, the ranking list of each ranked category varies by hours.  

We manually traversed screens and capture 3 to 5 screenshots with different functionalities and layouts in each downloaded app. There are 610 screenshots captured in total. Since UIs of apps in the same categories are highly comparable on layouts and contain quite similar icons, we thus discard most of the captured screens and finally keep 56 distinct screenshots with diverse categories and distinct icon types for user studies.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{Figs/Buttons.png}
    \caption{There are three types of buttons categorised by the contents of buttons. Button 1: with icon only; button 2: with text only; button 3: with both icon and text.}
    \label{fig_buttons}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figs/Image_Mosaic.jpeg}
    \caption{Illustrations of examples of mosaic application. After the mosaic processing, textual annotations of all icons on displayed UIs are cleared.}
    \label{fig_mosaic}
\end{figure*}

According to the content that appeared, buttons can be: icon button, text button and icon+text button. For example, `Button 1' of the screen in Fig. \ref{fig_buttons}, there is icon only, without any text description for its functionality. `Button 2' contains text only, with no icon appearing. `Button 3' contains both icon and text, the button thus can be activated by clicking either the text area or the icon area. However, during the UI exploration, we found that for the buttons with both text and icons, the text is somewhat unrelated to the icon patterns, where users cannot find the real functionalities of buttons replies on the icons only. To investigate the problem, we divided the 56 screens into two groups. Group 1 contains 41 screens, and most icons on these screens are icon+text buttons. We thus applied mosaic on the screens in Group 1 by covering the text part of icon+text buttons. As a result, there are icon buttons and text buttons on the screen. Fig.\ref{fig_mosaic} shows an example of a Mosaic application. Group 2 contains the rest of the 15 screens, where screens in this group contain no icon+text buttons. 
\begin{comment}


\begin{figure}
 \begin{subfigure}[]{.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Figs/fig_instruction_p1.png}
    \subcaption{}
  \end{subfigure}
  \hfill
  \begin{subfigure}[]{.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Figs/fig_instruction_p2.png}
    \subcaption{}
  \end{subfigure}
  \vfill
    \begin{subfigure}[]{.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Figs/fig_instruction_p3.png}
    \subcaption{}
  \end{subfigure}
  \hfill
    \begin{subfigure}[]{.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Figs/fig_instruction_p4.png}
    \subcaption{}
  \end{subfigure}
  \caption{Guidelines of user studies released for each user. }
  \label{fig_guideline}
  \vspace{-0.2in}
\end{figure}
\end{comment}

\begin{figure}
 \begin{subfigure}[t]{.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Figs/fig_test_case_p1.png}
    \subcaption{The first page for each UI, where users are required to select two icons on the displayed UI and drag the boxes with tags Q1 and Q2 to the corresponding icon area. Users then image the application scenarios of the displayed UI and propose an instance-level user intent for each selected icon.}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Figs/fig_test_case_p2.png}
    \subcaption{The second page for each UI, where users will see the textual annotations of icons which are hidden on the first page. Users are required to rate the alignment of the actual functionality of each selected icon with their expectations. }
  \end{subfigure}
  \vfill
    \begin{subfigure}[t]{.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Figs/fig_test_case_p3.png}
    \subcaption{The third page for each UI, where users are required to propose instance-level intents for two icons in the same way as the first page, based on the textual annotations instead.}
  \end{subfigure}

  \caption{An example of the interface for the user study.}
  \label{fig_test_case}
  \vspace{-0.2in}
\end{figure}

\subsection{Procedure}

All user studies are conducted online since that 50\% of our users are currently living in foreign countries, and hygiene policies of the Covid-19 pandemic are also applied to users who are living in the same country as us. All users have agreed to the policy that the dataset collected from users will be published together with their names, contact information, age group, living countries, spoken languages, and working positions.   

During each user study, we first presented a brief description of our research tasks to help users understand the goals of our user studies. We then provided the materials in the format of online slides for the user study and introduced the guidelines for providing answers on each slide. The slide for each user contains 17 test cases (excluding the pilot study, which contains 20 test cases). Each text case is about a distinct screenshot from the selected screen dataset. For the screens of group 1 where a subset of Mosaic screens is generated, the test case containing these screens includes 3 pages of slides. The mosaic version screen is displayed on the first page, where users are required to observe the presented mosaic version of screens and guess the functionalities of each icon (without any text description) based on their own experience. Users are prohibited to turn to the following pages to see the original version screens (with text descriptions) after they completed the first page. We asked users to imagine the scenario when they were interacting with the displayed screen and think about their aim/goal when they were going to click a certain button. According to the number of `Selection Frames', users then wrote down their goals about selected icons and dragged the related `Selection Frame' to its location on the screen area. After finishing the first page, users will see the original version of the Mosaic-modified screen on the second page. Compared with the original screen with visible text, users rated the alignment of each icon selected on the first page from 0 to 3, where 0 represents `Strongly Misaligned', 1 is for `Misaligned', 2 means `Aligned' and 3 is selected when users feel 'Strongly Aligned'. Next on the third page, users proposed intents on selected icons on the original version of screens with text visible. The rules of intent proposing are the same as the rules on the first page, where the only difference is that users can propose intents on selected icons referring to their textual contents.  

All user intents are in English. Users are encouraged to use multiple phrases for their expression, for example,` I wish to...', `I would like to...', `I'm going to...' etc. Fig.~\ref{fig_test_case} presents a test case with the 3 kinds of mentioned pages mentioned before. There are 3 versions of user studies and each version is released to 3 users. Before we started the official user studies, we first conducted a pilot study asking for feedback from a user with a special version of test cases. The pilot study contains 20 test cases, where users commented that the time is not sufficient for the considerate imagination of the application scenario of each screen. To deal with this issue, we thus reduce the test cases in each user study from 20 to 17, leaving more time for users to figure out UI content. The pilot study also received feedback that screens contained in adjacent test cases have similar functionalities. It is because we edited and inserted selected screenshots into test cases in the order of their default file names, which are highly dependent on the orders when they are captured from Apps. As the result, the captured screens with adjacent file names usually come from the same app or other apps in the same category. Thus, the selected screens displayed in the adjacent slides are likely generated from apps in the same categories, thus with similar icons displayed. We thus updated the order of each test case to reduce the overlapping icons between the adjacent test cases, and to avoid users proposing user intents similar to previous slides without figuring out the possible functionalities of icons in a certain UI content. The remaining 9 test cases are modified based on the feedback from the pilot study. 


==> 6-evaluation.tex <==
\section{Evaluation}
\label{section_e}

\subsection{Testing Dataset}
The testing dataset collected from the user study contains 752 distinct instance-level user intents, among which 34.3\% (258 of 752) are based on the screen after mosaic processing. For example, `This app is hard to use and I really need more instructions'; `I would like to share my current location with my friends'; `I would like to check my friends whose first name is Lucy', `I am really interested in this app and would like to know its background info', `I am interested in fashion and would like to dive deep into that category' and etc. The Word Cloud of the user intents is illustrated in Fig.~\ref{fig_user_intent_cloud}. As referred previously, all textual elements are removed manually from mosaic screens, and the areas of the removed textual elements are filled with the background color of the text, as shown in Fig.~\ref{fig_mosaic}, which is to evaluate the ability of our model to find the target buttons on screens without annotations. Among the user intents towards the mosaic screens, we also investigated the alignment of the actual functions regarded by users based on the annotations with the expectation of users. As shown in Fig.~\ref{fig_align}, there are 19.4\% of targeting buttons that are strongly misaligned with users' expectations and 12\% misaligned with the users' expectations. The buttons that are aligned and strongly aligned with the functionalities users think occupy 68.5\% of the buttons. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figs/fig_Cloud_user_intent_top100.png}
    \caption{The Word Cloud of the top 100 words in the collected user intents in the testing dataset.}
    \label{fig_user_intent_cloud}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/fig_align_pie_chart.png}
    \caption{The alignment of actual functionalities of selected buttons on the mosaic screen with the user's expectations.}
    \label{fig_align}
\end{figure}

\subsection{Testing Automation}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.2\textwidth]{Figs/fig_metrics.png}
    \caption{When the overlapping area of the output and the ground truth occupies more than 25\% of the output, the output is regarded as a correct result.}
    \label{fig_metrics}
\end{figure}

To evaluate the performance of our model automatically, we generated a testing dataset from the user intent provided by each user by labeling the ground truth areas relying on the area framed by users. Note that, since the text+icon button can be activated by both the icon and the text area, we label the whole text+icon button as the ground truth, if users frame the icon only or text area only of a certain button.

We also generated an evaluation agent which performs the comparisons between the output of our model with the ground truth of the testing dataset automatically. The method IoU (Intersection over Union), which is the ratio of the overlapping area of two areas over their union area, is a widely applied metric for measuring the accuracy of object detection tasks, thus is not applicable to our tasks, since the ground truth contains both text and icon area, while the output of our model may contain parts of that, i.e., the icon or text only. We thus propose a metrics that, the output (target operational area) of our model is verified as accurate if the overlapping area of our output is no less than 25\% area of the ground truth. An illustration is presented in Fig.\ref{fig_metrics}.showing the ground truth of the user content with id 710 in our testing dataset. The output of our model is also presented, which is verified as an accurate result since the overlapping area occupies more than 25\% areas of our output.

\subsection{Evaluating Capability of the Element Detector}

In our model, both Icon Classifier and  Descriptive-Word Classifier rely on the the graphic or textual elements detected by UIED. In other words, if the ground truth area cannot be detected by UIED, it will consequently be missed by our model. Thus the capacity of UIED on detecting elements significantly affect the performance of our model. However, UIED is equipped with customized GUI element detection methods perform well with customised configuration based on element scales on a certain screen, e.g. the size of the minimum GUI element on screens. For a batch of different screens, it is hard to find a general configuration for UIED to work with the best performance on each screen. For example, for a certain configuration of the minimum GUI element size, it may be relatively too small so that the UIED recognize partial patterns of buttons or background as an elements, while it is likely to be relatively too large so that the UIED miss many GUI elements on screens. The complexity of screen background also affects the accuracy of element detection by UIED.  With the configuration of UIED in our model, we investigated the ratio for testing datasets when the ground truth area of each user intent is among the elements detected by UIED on each corresponding screen. The ratio on the original screen dataset without the mosaic images is $77.85\%$ while the ratio on the Mosaic\_Positive dataset is $74.73\%$. We also tested the ratio on the testing dataset containing all user intents, the dataset containing all mosaic user intents and dataset contatining positive mosaic and negative mosaic user intents respectively, and the ratios on each of the mentioned dataset are $72.67\%$, $62.79\%$, $64.14\%$ and $65.71\%$. The ratio is shown as the green area in Fig.~\ref{fig_eva_1} and Fig.~\ref{fig_eva_2} on the relevant testing dataset domain.    


\subsection{Evaluating the End-to-End Operational Area Targeting}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/fig_Evaluation_1.png}
    \caption{The accuracy of our model on the Original Screen Dataset and the Mosaic\_Positive + Original Screen Dataset}
    \label{fig_eva_1}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/fig_Evaluation_2.png}
    \caption{The accuracy of our model on datasets with mosaic screens.}
    \label{fig_eva_2}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/fig_Evaluation_3.png}
    \caption{The accuracy of our model on the Original Screen Dataset and the Mosaic\_Positive + Original Screen Dataset compared with UIED\_Random Approaches.}
    \label{fig_eva_3}
\end{figure}

The user intents in the testing dataset can be grouped into two categories, one contains all user intents based on the original screens (without mosaic processing). Users are required to propose intents in this category based on their understanding of the whole screen, the recommended targeting area labeled by users thus can be regarded as the ground truth with high confidence. On the contrary, the other category contains user intents based on the mosaic screens, where all annotations are removed. The recommended operational area by users is thus mainly based on their own previous experience, without any reference to annotations. The strongly aligned and aligned user intents are thought to be close to the original annotations of these icons by users, and the recommended operational area of these user intents can also be regarded as the ground truth. However, user intents that are rated as misaligned and strongly misaligned indicate that in the opinion of participants, the recommended operational area in the previous pages cannot be treated as the ground truth. For evaluating the end-to-end operational areal targeting ability of our model, we thus first test our model on the original screens and the dataset of the original screens with strongly aligned and aligned mosaic screens (referred to as Mosaic\_Positive). Fig.~\ref{fig_eva_1}
demonstrates the evaluation results. Our model achieves $64.43\%$ on the original screen dataset, and archives $58.56\%$ on the Mosaic\_Positive + Original Screen Dataset. The season why the accuracy of our model decreases with the user intents on mosaic screens is that, all textual annotations are removed so that only CV techniques based UIED and the icon classifier can be adopted. We also compared the capability of our model with CV techniques only (do not consider textual elements detected by UIED) and the capability of our model with Text only (do not consider graphic elements detected by UIED). It can be seen in Fig.~\ref{fig_eva_1} that when the textual contents are ignored, the accuracy of the model on the original dataset is $32.11\%$ and the accuracy on the Mosaic\_Positive + Original Screen Dataset increased to $33.12\%$, which are roughly half of the correctness of our model. If only textual elements are considered while ignoring the graphic elements on screens, the accuracy on the original screen dataset is $48.78\%$ on the original dataset and drops to $38.15\%$ on the Mosaic\_Positive + Original Screen Dataset, since textual annotations about buttons are removed.

 We then evaluate the capability of our model on the testing dataset without annotations. Since the Text based techniques can not be adopted for searching the textual elements, the accuracy of our model on the three mosaic dataset thus decrease apparently compared with the accuracy on the testing dataset with the original screen + Mosaic\_Positive dataset. The negative mosaic data are also considered since they can reflect the practical scenarios where there existing many buttons whose functionalities are not aligned with users' expectations. It can be seen from Fig~\ref{fig_eva_2} that with the negative mosaic data, the accuracy of our models is $53.87\%$, where the CV technique only can accomplish $32\%$ of accuracy and the Text technique only can achieve $32.67\%$. For the dataset where all annotations of graphic elements are removed, our model achieves $33.72\%$ on the Mosaic\_Positive+Mosaic\_Negative, $38.62\%$ on the Mosaic\_Positive and $25.71\%$ on Mosaic\_Positive respectively, which are quite close to the approach with our CV techniques. The accuracy with Text technique only approach is around $0\%$. The reason why the accuracy is a little bit above $0\%$ is that, there are some text buttons remaining on the screen, which are the ground truth for these correctly processed user intents.

To test the usability of our model, we compare the performance of our model with a random algorithm that randomly selects a certain number of elements from elements detected by UIED. We use the random algorithm to simulate the situation when a user does not know the targeting operational area and randomly explored buttons on the screen. We use the number `x' with UIED\_Random\_x denotes the maximum number of randomly selected elements of the approach to cover the targeting area. Fig.~\ref{fig_eva_3} shows the accuracy of each approach, which also indicates the possibility to cover the targeting operational area when randomly selecting a certain number of elements. The results illustrate that our model significantly overpasses the random approaches.


 

==> 7-discussions.tex <==
\section{Discussion}

The GUI element detector plays a key role in providing targeting element candidates for user intents as shown in Section~\ref{section_e}, where the performance of candidate detection significantly limits the accuracy of our model on the testing dataset. To the best of our knowledge, there are no existing GUI detection tools designed for a batch of general UIs with different scales. The dependence on the capability of existing tools is not only the shortage for our approach, but also the shortage for all pipeline-based approaches. But in theory, the performance of our model would be improved with a more capable GUI detection tool. Besides, many icons serve as decorations only, instead of acting as indicators for certain functionalities. They have quite different appearances from the user's expectation, where fig.~\ref{fig_align} can indicate it, which also significantly limits the accuracy of our model on the testing dataset, especially for UIs without any textual annotation. This is also one of the shortages of our approach, but it could be easily improved by feeding more icons with customized styles into the CNN icon classifier of the pipeline.

There are various application scenarios for our approach.  For example, it provides services of smartphones to people who are unfamiliar with smartphones, not convenient to use smartphones and even have no knowledge of using a smartphone, such as the older generation and people with disability. Although they may not be clear about the exact actions required for their intents, users can easily interact with the smart devices by describing their situation, which is also a strong motivation for our approach to process instance-level user intents. Another benefit it can provide is to save exploration time for desired functionalities. When smartphone users are unfamiliar with an app, finding a certain functionality usually requires some time for users to investigate the capabilities of an app by trying different buttons, especially when UIs contain a large number of complicated components and annotations. With the help of our approach, users can quickly find the targeting area within 2 seconds. 

On the aspect of machine learning technology, our approach achieves a great breakthrough for providing a bridge between linguists and computer visions, by translating instance-level user intents into a precise operating area on UIs. The model in this paper can be directly adopted for generating training data for the convergence of Computer Vision (CV) and Natural Language Processing (NLP). 

 

\section{Conclusion}
In this paper, we explored the capability augmenting of virtual assistants via the precise operational area targeting on UIs for tackling instance-level user intents. We proposed a novel cross-modal pipeline combining the natural language processing technique and computer vision techniques with a novel cross-modal bridging approach. We also collected a dataset with instance-level user intents and precise operational areas on UIs from a group of diverse mobile users for testing automation. The accuracy on the testing dataset of our model is $64.43\%$, which demonstrates that our approach can accurately and thoroughly understand instance-level user instants and find the precise operational area without metadata. It also presents that our approach successfully achieves the goal of requiring zero-effort from developers and end-users, handling custom and UI-level tasks and can be adapted for any category of apps.





==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

